On Multi-Modal Learning of Editing Source Code

In recent years, Neural Machine Translator (NMT) has shown promise in automatically editing source code. Typical NMT based code editor only considers the code that needs to be changed as input and suggests developers with a ranked list of patched code to choose from - where the correct one may not always be at the top of the list. While NMT based code editing systems generate a broad spectrum of plausible patches, the correct one depends on the developers' requirement and often on the context where the patch is applied. Thus, if developers provide some hints, using natural language, or providing patch context, NMT models can benefit from them. As a proof of concept, in this research, we leverage three modalities of information: edit location, edit code context, commit messages (as a proxy of developers' hint in natural language) to automatically generate edits with NMT models. To that end, we build MODIT, a multi-modal NMT based code editing engine. With in-depth investigation and analysis, we show that developers' hint as an input modality can narrow the search space for patches and outperform state-of-the-art models to generate correctly patched code in top-1 position.

==> tables/other-examples.tex <==

\begin{figure}[!t]
\small
\centering

\rule{\linewidth}{0.7pt}
\flushleft \tick ~Example 1 : External guidance can \textbf{characterize edit type}. \\

\begin{subfigure}{0.95\linewidth}
\caption{Code Before Editing}
\begin{tabular}{l}
\lstset{escapechar=~,style=CustomJava}
\begin{lstlisting}
@java.lang.Override 
public void setSpeed (double speed) { 
  for(int i = 0; i < ~\red{\textbf{(motors.size()-1)}}~; i++){ 
      motors.get(i).set(speed);
  }
} 
\end{lstlisting}
\end{tabular}
\end{subfigure}

\begin{subfigure}{0.95\linewidth}
\caption{Code After Editing}
\begin{tabular}{l}
\lstset{escapechar=~,style=CustomJava}
\begin{lstlisting}
@java.lang.Override 
public void setSpeed (double speed) { 
  for(int i=0; i < ~\dkgreen{\textbf{motors.size()}}~; i++){ 
      motors.get(i).set(speed);
  }
} 
\end{lstlisting}
\end{tabular}
\end{subfigure}
\quad {\bf Edit Guidance:} Fixed \textbf{\red{indexing errors}} and velocity calculation

\rule{\linewidth}{0.7pt}
\flushleft \tick ~Example 2 : External guidance can \textbf{exactly say} what the edit should be. \\
\begin{subfigure}{0.95\linewidth}
\caption{Code Before Editing}
\begin{tabular}{l}
\lstset{escapechar=~,style=CustomJava}
\begin{lstlisting}
public Cards.Card draw() { 
    return this.deck.remove(0); 
} 
\end{lstlisting}
\end{tabular}
\end{subfigure}

\begin{subfigure}{0.95\linewidth}
\caption{Code After Editing}
\begin{tabular}{l}
\lstset{escapechar=~,style=CustomJava}
\begin{lstlisting}
public Cards.Card draw() { 
    ~\dkgreen{\textbf{if (deck.size() > 0) \{}}~
        return this.deck.remove(0); 
    ~\dkgreen{\textbf{\}}}~
    ~\dkgreen{\textbf{else return null;}}~
} 
\end{lstlisting}
\end{tabular}
\end{subfigure}
\quad {\bf Edit Guidance:} Fix bug with \red{\textbf{empty deck}}
\rule{\linewidth}{0.7pt}

\flushleft \tick ~Example 3 : Context may help choose \textbf{right identifier} \\
\begin{subfigure}{0.95\linewidth}
\caption{Code Before Editing}
\begin{tabular}{l}
\lstset{escapechar=~,style=CustomJava}
\begin{lstlisting}
public void setPredecessor (model.Message m) { 
  this.predecessor = Integer.valueOf(m.Content);
  model.Message sent = new model.Message(); 
  sent.To = m.Origin; 
  sendMessage(~\color{red}\textbf{m}~); 
}
\end{lstlisting}
\end{tabular}
\end{subfigure}

\begin{subfigure}{0.95\linewidth}
\caption{Code After Editing}
\begin{tabular}{l}
\lstset{escapechar=~,style=CustomJava}
\begin{lstlisting}
public void setPredecessor (model.Message m) { 
  this.predecessor = Integer.valueOf(m.Content);
  model.Message ~\dkgreen{\textbf{sent}}~ = new model.Message(); 
  sent.To = m.Origin; 
  sendMessage(~\dkgreen{\textbf{sent}}~); 
}
\end{lstlisting}
\end{tabular}
\end{subfigure}
\quad {\bf Edit Guidance:} Fix bug of \textbf{\red{sending wrong message}}
\rule{\linewidth}{0.7pt}

% \caption{Examples motivating the design choices of robust code change generator. First, additional guidance (often in form a review) can drive code editor, helping generate more precise edits. Second, when the guidance exactly says what to do, the tool still needs to generate syntactically and semantically correct code. And finally, the context of the code edit location help choose proper tokens.}
\label{fig:motivating}
\end{figure}

==> todo.tex <==
1. Add acknowledgement section. 


% \section*{Response to the meta-reviews from ASE}


% % \subsection*{Required TODO}
% {\it The reviewers all agree that the work is promising but there are several weak points that need to be addressed before final acceptance. The weak points include:}

% {\color{blue} We thank the reviewers for their valuable comments and feedback on our work. In this version, we addressed the required TODOs mentioned in the meta-review, as per ASE guidelines. We annotated this manuscript highlighting the changes in \blue{blue}. 
% % Note that, in this revision, we added line number and page number for quick referencing between review comment and actual change. In the camera ready version, we will abide by the formatting requirement of ASE. 
% We are working on addressing other comments in the detailed reviews, which we hope to submit with the camera-ready version of the paper.}
% %Our response to the comments in meta review are as follow.}
% %We sincerely hope this version of the paper is acceptable.}

% \begin{enumerate}
%     \item {\it Clarify the modalities claim. Currently, the authors refer to three modalities, but the context and the lines can be considered as the same modality, i.e., both are represented in code.}
    
%     {\color{blue}
%     % - \Cref{sec:tool} - 224
%     - Thanks for this comment. We do acknowledge that code to be edited is essentially a substring of the context presented. However, by extracting such code, we provide MODIT with additional information about the change location. Thus, we prefer to consider ``code needs to be edited" as a separate mode of information (i.e., modality) indicating change location than code context. We clarified this point in Section-I, at the beginning of Section-III, and the experimental design of RQ2 (Section-V).
%     }
    
%     \item {\it Clarify or or remove claims of significance. When the paper claims that MODIT 'generates significantly more correct patches than models trained from scratch', the paper should back up that claim.}
    
%     {\color{blue} 
%     % - \Cref{sec:results} - RQ1 result(470-474), RQ2 lessons 1 (627-631).
%     - Thanks for this comment; We apologize for the misunderstanding. Our improvement comes from two design choices: 
    
%     \begin{itemize}
%         \item RQ1: pre-training vs. training from scratch: Our empirical results show that results are {\em significantly} improved when we use a pre-trained model, in contrast to a model trained from scratch for code editing (see Table-II). We have clarified this point in RQ1.
%     % ~\rayb{give line numbers}
%     \item RQ2: multi-modality: We have reworded our claim (see lessons learned), saying each of the modalities contribute to some extent to improve the overall performance (Section-V). 
%     % ~\rayb{give line numbers}
%     \end{itemize}
    
    
    
    
%     .
%     }
    
%     \item {\it Re-write the related work. Related work section has too many links, and does not really compare and contrast previous work with this paper. The authors should remove some citations and also have a more in-depth discussion of the related work. Every related work should be presented in relation to the work of this paper.}
    
%     {
%     \color{blue}
%     - Thanks for the suggestion. We have reorganized the related work putting more emphasis on the insights from existing works in the literature. 
%     }
    
% \end{enumerate}


% % \subsection*{Additional Changes}
% % \begin{itemize}
% %     \item \textbf{{\color{red}[Must - Writing]} R1.} The writeup for RQ2 could be more clear. Table III is difficult to parse. 
    
% %     {\color{blue}- RQ2 (555-563).}
    
% %     \item \textbf{{\color{red}[Must - Writing]} R2.} One of the novelty of the proposed approach is to involve the commit messages. But as we know, developers usually write commit messages after the code editing. Writing commit messages as guidance for code editing may cost developers’ time and efforts. Also, it cannot be guaranteed that the guidance is exactly clear before the code editing. Such concern may hinder the practicability of the proposed approach.
    
% %     {\color{blue} - \Cref{sec:threats} (843-853).}
    
% %     \item \textbf{{\color{orange}[Maybe - Exp]} R2.} In Tufano et al.’s work [8], different beam sizes are experimented. Since the beam search size can impact the computed accuracy, it would be better to test the results with different beam search sizes.
% %     \item \textbf{{\color{orange}[Maybe - Exp]} R2.} In Section VI-A, reporting the location prediction accuracy and comparing with the baseline approaches can make the answer more convincing and comprehensive.
    
% %     \item \textbf{{\color{orange}[Maybe - Exp]} R3.} The paper does not provide results in terms of syntax correctness of the code editing suggestions. Approaches like CODIT can guarantee syntax correctness of the suggestions, while the proposed approach does not. For this reason, it would be important to provide empirical evidence that MODIT can actually suggests syntactically correct code in most cases. Additionally, while I agree that the top-1 suggestion is the most interesting one and recommendation system should focus on the top-k suggestions the authors should provide an idea of how are the results outside the top-1.
    
% % \end{itemize}
% % % \pagebreak
